On Replacing Cryptopuzzles with Useful Computation in Blockchain Proof-of-Work Protocols

Proof-of-Work (PoW) blockchains have emerged as a robust and effective consensus mechanism in open environments, leading to widespread deployment with numerous cryptocurrency platforms and substantial investments. However, the commonly deployed PoW implementations are all based on solving cryptographic puzzles. Researchers have been pursuing the compelling idea of replacing cryptopuzzles with useful computing tasks for over a decade, in face of the substantial computational capacity of blockchain networks and the global pursuit of a more sustainable IT infrastructure. In this study, we conduct a comprehensive analysis of the prerequisites for alternative classes of tasks. We provide insight into the effect of introducing "usefulness" and of transitioning to task classes other than cryptopuzzles. Having distilled the prerequisites, we use them to examine proposed designs from existing literature. Finally, we discuss pertinent techniques and present research gaps in the current state-of-the-art.

==> tables/table_approaches.tex <==
% TABLE TO SUMMARIZE BPP, BTP and interface primitives

\begin{table}
\tiny
\centering
\caption{List of the identified approaches and their applicability to k-Orthogonal Vector (k-OV), Traveling Salesman Problem (TSP) and Machine Learning (ML) tasks: Applicable(A), Open (O), Not Applicable (NA). List of properties and aspects that the approaches may affect either in a positive or negative way.}
\label{table:approaches}

\begin{tabular}{p{2.5cm}p{0.7cm}p{0.7cm}p{0.7cm}p{3cm}p{3cm}} 

\toprule
     \bf Approach & 
     \bf k-OV &
     \bf TSP &
     \bf ML &
     {\bf Advantages} &
     {\bf Disadvantages} \\
\toprule

{\specialcell[]{Polynomial transformation}} & 
A & 
O & 
O &
{\it BT hardness, Context sensitivity, Strong usefulness} &
{\it Non-zero variability across BTs, Proposal Fairness} \\ 

\midrule

{\specialcell[]{Shuffling service}} & 
A & 
A & 
A &
{\specialcell[]{Collusion attacks \\ \it Context Sensitivity}} &
{\specialcell[]{Bandwidth req.}} \\ 

\midrule

{\specialcell[]{Watermarking}} & 
O & 
O & 
A &
{\specialcell[]{\it Context sensitivity}} &
{\specialcell[]{ Untested safety}} \\ 

\midrule

{\specialcell[]{Meaningful nonce}} & 
O & 
A & 
A &
{\specialcell[]{\it Context sensitivity \\ \it Strong usefulness}} &
{\specialcell[]{ Untested safety}} \\ 

\toprule

\end{tabular}
\end{table}

